Reinforcement Learning as an Improvement Heuristic for Real-World Production Scheduling

The integration of Reinforcement Learning (RL) with heuristic methods is an emerging trend for solving optimization problems, which leverages RL's ability to learn from the data generated during the search process. One promising approach is to train an RL agent as an improvement heuristic, starting with a suboptimal solution that is iteratively improved by applying small changes. We apply this approach to a real-world multiobjective production scheduling problem. Our approach utilizes a network architecture that includes Transformer encoding to learn the relationships between jobs. Afterwards, a probability matrix is generated from which pairs of jobs are sampled and then swapped to improve the solution. We benchmarked our approach against other heuristics using real data from our industry partner, demonstrating its superior performance.

==> sec/related_work.tex <==
% Related Work - Learning Improvement Heuristic, im Kontext anderer komb. Optimierungsprobleme
%     - Learning 2-opt Heuristics for the Traveling Salesman Problem 
%     via Deep Reinforcement Learning: \cite{Costa2020}
%     Recent works using deep learning to solve the Traveling Salesman Problem (TSP) have
%     focused on learning construction heuristics. Such approaches find TSP solutions of good
%     quality but require additional procedures such as beam search and sampling to improve
%     solutions and achieve state-of-the-art performance. However, few studies have focused on
%     improvement heuristics, where a given solution is improved until reaching a near-optimal
%     one. In this work, we propose to learn a local search heuristic based on 2-opt operators via
%     deep reinforcement learning. We propose a policy gradient algorithm to learn a stochastic
%     policy that selects 2-opt operations given a current solution. Moreover, we introduce a
%     policy neural network that leverages a pointing attention mechanism, which unlike previous
%     works, can be easily extended to more general k-opt moves. Our results show that the
%     learned policies can improve even over random initial solutions and approach near-optimal
%     solutions at a faster rate than previous state-of-the-art deep learning methods.
%     - "MGRO \cite{Hao2021} learns a policy to aid iterated greedy, an improvement heuristic, to solve the hybrid flow shop scheduling problem." \cite{Zhang2022}
%     - "As the first neural improvement heuristic, NeuRewriter [11]
%     learns to pick local search operations and rewrite the local
%     components of the current solution. It successfully outperformed the neural construction solver AM [9] and Nazari
%     et al. [8] on solving CVRP. The L2I framework proposed in Lu
%     et al. [73] explored the hybrid of learning framework and
%     conventional methods. It used a learning‐based neural network
%     to select local search operators from a candidate pool containing several professional local search operators and became
%     the first neural solver to outperform hand‐crafted LKH3
%     solver [176] on solving CVRP instances in terms of the solution quality (though required longer computation time). By
%     exploring SA heuristics as well as the idea of the large neighbourhood search (LNS) heuristics which considers applying
%     destroy and repair operators to current solutions, the neural
%     LNS (NLNS) was proposed in Hottung et al. [71] and also
%     showed superior performance over AM [9]. Wu et al. [2]
%     proposed a Transformer‐based improvement solver for TSP
%     and CVRP. By learning to perform the pair‐wise operators (e.g.
%     2‐opt, reinsert, or swap as illustrated in Figure 2), it has shown
%     a promising result over NeuRewriter [11] and AM [9]. The
%     method of Wu et al. [2] was then improved to dual‐aspect collaborative transformer (DACT) method by Ma et al. [70]
%     based on a upgraded deep model and a CL strategy to enhance
%     the RL. Though DACT displayed a significantly better inference and generalisation performance than Wu et al. [2], its
%     computational efficiency is still not satisfactory when
%     compared to the latest neural construction solvers (e.g. POMO
%     [10]). In a more recent work, DACT was further modified to
%     N2S [72] to solve the pickup and the delivery problems
%     (PDPs). By further equipped with a designed data augmentation scheme similar to POMO [10], N2S significantly outperformed DACT, Heter‐AM [155], and POMO on solving
%     PDPs and became the first learning‐based solver to outstrip
%     the well‐known hand‐crafted LKH3 solver [176] on synthesised PDP datasets." \cite{Zhang2022}
